TraCE: Trajectory Counterfactual Explanation Scores

Counterfactual explanations, and their associated algorithmic recourse, are typically leveraged to understand, explain, and potentially alter a prediction coming from a black-box classifier. In this paper, we propose to extend the use of counterfactuals to evaluate progress in sequential decision making tasks. To this end, we introduce a model-agnostic modular framework, TraCE (Trajectory Counterfactual Explanation) scores, which is able to distill and condense progress in highly complex scenarios into a single value. We demonstrate TraCE's utility across domains by showcasing its main properties in two case studies spanning healthcare and climate change.

==> changes_to_make.tex <==

From Ed:
[ ] update figure 1 to include corrections;
[ ] make sure typos are fixed in equations and methodology;
[X] add a little more context;
move theorem 1 to the preliminaries and add some context;
[ ] alter the proof in the appendix to reflect the vectors being agnostic to space.

[X] Add extra ICU examples (neg 28? pos ?)
[X] Finish tidying up the plots
[ ] Add extra SSP example (Poland?)
[X] Add Welch's t-test result
[X] Include link to repo

[X] Ed's suggestions for improving clarity in the ICU case study: "My idea was to:
   [X] stack the probability and TraCE plots vertically so that they share the same x axis. That would make it VERY clear as to which time points line up with which.
   [X]We should then also lock the y axis for -1 to 1 for TraCE
   [X] 0-1 for the probability plot,
   [X] x-axis from 0 to last time point for both plots
   [X] add a horizontal dotted black line at y=0 on the TraCE plot
   [X] remove the top and right borders of the plot. 
   [X] I often find that using plt.style.use('seaborn-paper') or something similar gets my plots looking twice as nice with practically 0 effort. Feel free to play around with some of the different styles. Putting that line in the code will change the default format for all the plots."
   [X] Change TraCE y ticks (1.0, 0.5, 0...)

Area Chair xeLt
*Ed* [X] there is room for improvement in the clarity of the methodology and notations
Ed/Jeff [X] inclusion of more explanations/examples


Reviewer VKpP

*Ed* [] description of R2 is quite confusing

All questions are related to section 3:

*Ed* [X] Theorem 1 would be better placed in the preliminaries section.
Resolution: "We will make this change and look to place Theorem 1 at the end of the notations section. It will be accompanied by additional context to avoid the theorem looking too abstract."

*Ed* [X] Vector has not a fixed location in space. In this way, the statement of the Theorem 1 is inaccurate.
"We agree with this, and adding this clarification makes Theorem 1 precise. We will also include this clarification in the proof in Appendix A."

*Ed* [ ] R1 definition clarification
"We will clarify this in the paper as..." in rebuttal

*Ed* [X] R2 x't+1 was not previously defined, and so it is not clear if the formulation considers a single target or one for each xt.
Update equation

*Ed* [X] R2:  The way R2 was defined, the conclusions w.r.t. R2=1 when... are not correct.

Jeff/Ed [ ] More discussion is required to clarify why the proposed scores R1 and R2 are good options to solve the problem.


Reviewer 8AhG

-Jeff- [X] The section describing the TraCE scores is quite brief and it could be helpful to provide more explanations/examples to make it easier for readers to follow, e.g. by relating variables such as xt and x' to the healthcare example in the introduction. Further, there are some unclarities in Section 3:

*Ed* [X] in Figure 1,  is defined as (the reviewer assumes) the absolute value of an angle. However, in the same figure, the range is given as [-1, 1] (and not [0, 1]). It is not clear why this is.
-in Figure 1, R2 is indicated as the angle between v and v* (not v^ and v* as the equation indicates).
-for the computation of the mean TraCE in Figure 1, should it be the sum m+n in the denominator (or is the product correct)?
"We recognise that Figure 1 contains these errors, which are now rectified. We will also include subscripts in the figure for alignment with the mathematics."

*Ed* [ ] the text states that you want to measure the distance travelled relative to the angle size R2, can you elaborate on this and relate it to the equations?
Us to provide clarity as in the rebuttal

*Ed* [X] are the subscripts in the expression for vt* in relation to equation (4) correct? Or should it be vt* = xt' - xt+1? It could be beneficial to include subscripts for the ""s in Figure 1.
"This is an error; we will correct this in the paper."

-Jeff- [X] In Section 4.1.4.1, it is not clear what the input/output to the MLP is (from experiment results, it can seem like input/output are individual time steps, but this is not really clear). Further, the use of an MPL with only two hidden layers is not commented on. And why is the MLP trained for a maximum of only 10 iterations? Or should it be 10 epochs?
"You are correct: the input to the MLP is an individual patient timestep and the outputs are class probabilities. We used two hidden layers and trained over 10 epochs as this balanced performance with risk of overfitting. We will address all of this in the paper"

-Jeff- [X] Could the authors also comment on the use of the TraCE framework in a bigger neural network?
"TraCE summarises scenarios into an easily interpretable score. Its utility will become more evident with more complex scenarios, such as those warranting a larger neural network. We will comment on this."

-Jeff- [X] In Figure 2, there are a different number of ICU stay timepoints in (a) and (b), which makes comparison difficult (same for Figure 6 in the appendix). Is it possible from this plot to say that the TraCE scores increase prior to the classifier probabilities?
"We agree that the timepoint mismatch makes comparison difficult. TraCE scores do increase prior to the classifier probabilities when plotting on a shared time axis. We will update these figures."

-Jeff- [X] Is the model (MLP) used in the climate example the same as the one used in the health example?
"The climate scenarios are not generated by a machine learning model. Instead, we use SSP projection datasets produced by physics-driven CMIP6 climate models. SSPs are considered in turn, against which observations are compared for corresponding time steps. We will clarify this."

-Jeff- [X] Are the previous time steps considered when computing the TraCE score for the next decision?
"The TraCE score for a given time step considers the single previous one. We present scores in two forms: raw instantaneous (ICU study); average and cumulative (SSP study). We have recognised opportunities to explore approaches such as computing score gradients or integrals through successive time steps, or time-dependent score weighting."


Reviewer Qqh1
-Jeff- [X] The experiment section simply lists the difference in figure without any high-level understanding. Namely, what we can after we observe the so called counterfactual score in real time?
"Our case studies aim to demonstrate various ways in which real-time TraCE scores can help inform human decision-making, without the need for background domain understanding in order to read the scoring results. For both studies, domain expertise are required prior to deployment: the presented results are for demonstration purposes only.
In the ICU study, TraCE scores could aid clinicians with early detection of patient deterioration, to inform and improve quality of care. For the climate study, TraCE scores could help stakeholders monitor the development of regions against established pathways.
While we highlight some results, we do not draw conclusions about their implications. We believe that detailed interpretation first requires engagement with domain experts to ensure robust deployment of TraCE. This is beyond the scope of this paper, which introduces the technique.
We will address these considerations in the manuscript."

-Jeff- [X] The content in Section 2 is very similar to the definition of adversarial samples, some discuss or connection with adversarial samples would be interesting.
"We agree on the similarity between counterfactual explanations and adversarial samples. We will acknowledge this connection in the manuscript with appropriate references to established studies."

-Jeff- [X] (1) Ablation study with regard to the trade-off parameter \lambda is very important for comprehensively understanding the proposed method.
"The appropriate  value varies by application and intended purpose of implementation. We expect tuning to consider domain expertise, since  affects interpretation of the resulting score. Given that this manuscript introduces the technique with purely demonstrative case studies, and that we are already limited on space with the excellent reviewer feedback, we suggest simply highlighting in the paper the importance of choosing a suitable value for \lambda."

-Jeff- [X] (2) It is highly interesting if any interaction between the human and decision making process after we obtain the counterfactual score.
"We are working towards a separate study assessing how interactions with explainable AI systems changes the decision-making process of clinicians. For the current manuscript, we focus on the technical introduction of the TraCE method, with inclusion of two example applications demonstrating the technique. Without significant input from domain expertise we feel it would be inappropriate to emphasise the specific initial results, given that they are presented purely as a demonstration of the technique. We will clarify this in the manuscript, alongside future work."
